Disentangling a dynamical Higgs

The pattern of deviations from Standard Model predictions and couplings is different for theories of new physics based on a non-linear realization of the $SU(2)_L\times U(1)_Y$ gauge symmetry breaking and those assuming a linear realization. We clarify this issue in a model-independent way via its effective Lagrangian formulation in the presence of a light Higgs particle, up to first order in the expansions: dimension-six operators for the linear expansion and four derivatives for the non-linear one. Complete sets of pure gauge and gauge-Higgs operators are considered, implementing the renormalization procedure and deriving the Feynman rules for the non-linear expansion. We establish the theoretical relation and the differences in physics impact between the two expansions. Promising discriminating signals include the decorrelation in the non-linear case of signals correlated in the linear one: some pure gauge versus gauge-Higgs couplings and also between couplings with the same number of Higgs legs. Furthermore, anomalous signals expected at first order in the non-linear realization may appear only at higher orders of the linear one, and vice versa. We analyze in detail the impact of both type of discriminating signals on LHC physics.

==> Fdiagrams/WWhh_F.tex <==

\begin{fmffile}{WWhh_fer}
$i\mathcal{A}=$
\parbox{4.5cm}{\centering
\begin{fmfgraph*}(100,80)

\fmfleft{i1,i2}
\fmfright{o2,o1}
  \fmf{boson,label=$p_-$,l.side=left}{i2,v1}
  \fmf{boson,label=$p_+$,l.side=left}{i1,v1}
  \fmf{dashes,label=$p_1$,l.side=right}{v1,o1}
  \fmf{dashes,label=$p_2$,l.side=right}{v1,o2}
  
\fmfv{lab=$W^+_\mu$,l.angle=180}{i2}
\fmfv{lab=$W^-_\nu$,l.angle=180}{i1}
\fmfv{lab=$h$,l.angle=0}{o1}
\fmfv{lab=$h$,l.angle=0}{o2}
\end{fmfgraph*}}
 

\end{fmffile}


==> Fdiagrams/WWhh_G.tex <==

\begin{fmffile}{WWhh_gauge}
$i\mathcal{A}=$
\parbox{4.5cm}{\centering
\begin{fmfgraph*}(100,80)

\fmfleft{i1,i2}
\fmfright{o2,o1}
  \fmf{boson,label=$p_-$,l.side=left}{i2,v1}
  \fmf{boson,label=$p_+$,l.side=left}{i1,v1}
  \fmf{dashes,label=$p_1$,l.side=right}{v1,o1}
  \fmf{dashes,label=$p_2$,l.side=right}{v1,o2}
  
\fmfv{lab=$W^+_\mu$,l.angle=180}{i2}
\fmfv{lab=$W^-_\nu$,l.angle=180}{i1}
\fmfv{lab=$h$,l.angle=0}{o1}
\fmfv{lab=$h$,l.angle=0}{o2}
\end{fmfgraph*}}
+
\parbox{4.5cm}{\centering
\begin{fmfgraph*}(100,80)

\fmfleft{i1,i2}
\fmfright{o2,o1}
  \fmf{boson,label=$p_-$,l.side=left}{i2,v1}
  \fmf{boson,label=$p_+$,l.side=left}{i1,v2}
  \fmf{boson,label=$W,,\: k$}{v1,v2}
  \fmf{dashes,label=$p_1$,l.side=right}{v1,o1}
  \fmf{dashes,label=$p_2$,l.side=right}{v2,o2}
  
  \fmfv{lab=$\alpha$}{v1}
  \fmfv{lab=$\beta$}{v2}
%   \fmfv{lab=$\Bigg\downarrow \: q$,l.angle=-45,l.dist=10}{v1}
\fmfv{lab=$W^+_\mu$,l.angle=180}{i2}
\fmfv{lab=$W^-_\nu$,l.angle=180}{i1}
\fmfv{lab=$h$,l.angle=0}{o1}
\fmfv{lab=$h$,l.angle=0}{o2}
\end{fmfgraph*}}
+
\parbox{4.5cm}{\centering
\begin{fmfgraph*}(100,80)

\fmfleft{i1,i2}
\fmfright{o2,o1}
 \fmf{boson,label=$p_-$,l.side=left}{i2,v1}
  \fmf{boson,label=$p_+$,l.side=left}{i1,v2}
  \fmf{boson,label=$W,,\: k$}{v1,v2}
  \fmf{dashes,label=$p_2$,l.side=right}{v1,o1}
  \fmf{dashes,label=$p_1$,l.side=right}{v2,o2}
  
  \fmfv{lab=$\alpha$}{v1}
  \fmfv{lab=$\beta$}{v2}
%   \fmfv{lab=$\Bigg\downarrow \: q$,l.angle=-45,l.dist=10}{v1}
\fmfv{lab=$W^+_\mu$,l.angle=180}{i2}
\fmfv{lab=$W^-_\nu$,l.angle=180}{i1}
\fmfv{lab=$h$,l.angle=0}{o1}
\fmfv{lab=$h$,l.angle=0}{o2}
\end{fmfgraph*}}


\end{fmffile}


==> Fdiagrams/ZZh_bis.tex <==

\begin{fmffile}{zzh_biscoupl}
\begin{fmfgraph*}(50,50)

\fmfleft{i1,i2,i3}
\fmfright{o3,o2,o1}
  \fmf{dashes}{i2,v1}
  
\fmfv{lab=$Z_\mu$,l.angle=0}{o1}
\fmfv{lab=$Z_\nu$,l.angle=0}{o3}
\fmfv{lab=$h$}{i2}
\end{fmfgraph*}
\end{fmffile}


==> Fdiagrams/duWZ.tex <==

\begin{fmffile}{duWZcoupl}
\begin{fmfgraph*}(50,50)

\fmfleft{i1,i2}
\fmfright{o2,o1}
  \fmf{fermion}{i2,v1,i1}
  \fmf{boson}{v1,o1}
  \fmf{boson}{v1,o2}
  
\fmfv{lab=$Z_\mu$,l.angle=0}{o1}
\fmfv{lab=$W^+_\nu$,l.angle=0}{o2}
\fmfv{lab=$U_i$,l.angle=180}{i1}
\fmfv{lab=$D_j$,l.angle=180}{i2}
\end{fmfgraph*}
\end{fmffile}


==> Fdiagrams/duWh.tex <==

\begin{fmffile}{duWhcoupl}
\begin{fmfgraph*}(50,50)

\fmfleft{i1,i2}
\fmfright{o2,o1}
  \fmf{fermion}{i2,v1,i1}
  \fmf{dashes}{v1,o1}
  \fmf{boson}{v1,o2}
  
\fmfv{lab=$h$,l.angle=0}{o1}
\fmfv{lab=$W^+_\mu$,l.angle=0}{o2}
\fmfv{lab=$U_i$,l.angle=180}{i1}
\fmfv{lab=$D_j$,l.angle=180}{i2}
\end{fmfgraph*}
\end{fmffile}


==> Fdiagrams/hhhh.tex <==
\begin{fmffile}{hhhhcoupl}
\begin{fmfgraph*}(50,50)

\fmfleft{i1,i2}
\fmfright{o2,o1}
  \fmf{dashes,label=$p_{h1}$}{i2,v1}
  \fmf{dashes,label=$p_{h2}$}{i1,v1}
  \fmf{dashes,label=$p_{h3}$,l.side=right}{v1,o1}
  \fmf{dashes,label=$p_{h4}$,l.side=right}{v1,o2}
  
\fmfv{lab=$h$,l.angle=0}{o1}
\fmfv{lab=$h$,l.angle=0}{o2}
\fmfv{lab=$h$,l.angle=180}{i1}
\fmfv{lab=$h$,l.angle=180}{i2}
\end{fmfgraph*}
\end{fmffile}


==> Fdiagrams/hhqq.tex <==

\begin{fmffile}{hhqqcoupl}
\begin{fmfgraph*}(50,50)

\fmfleft{i1,i2,i3}
\fmfright{o3,o2,o1}
  \fmf{dashes}{i1,v1}
  \fmf{dashes}{i3,v1}
  \fmf{fermion}{o1,v1,o3}
  
\fmfv{lab=$h$,l.angle=180}{i1}
\fmfv{lab=$h$,l.angle=180}{i3}
\fmfv{lab=$f_\alpha$,l.angle=0}{o1}
\fmfv{lab=$f_\beta$,l.angle=0}{o3}
\end{fmfgraph*}
\end{fmffile}


==> Fdiagrams/qqZh.tex <==

\begin{fmffile}{qqZhcoupl}
\begin{fmfgraph*}(50,50)

\fmfleft{i1,i2}
\fmfright{o2,o1}
  \fmf{fermion}{i2,v1,i1}
  \fmf{dashes}{v1,o1}
  \fmf{boson}{v1,o2}
  
\fmfv{lab=$h$,l.angle=0}{o1}
\fmfv{lab=$Z_\mu$,l.angle=0}{o2}
\fmfv{lab=$U(D)_i$,l.angle=180}{i1}
\fmfv{lab=$U(D)_j$,l.angle=180}{i2}
\end{fmfgraph*}
\end{fmffile}


==> Fdiagrams/qqqq.tex <==

\begin{fmffile}{qqqqcoupl}
\begin{fmfgraph*}(50,50)

\fmfleft{i1,i2}
\fmfright{o2,o1}
  \fmf{fermion}{i2,v1,i1}
  \fmf{fermion}{o1,v1,o2}
  
\fmfv{lab=$q_n$,l.angle=0}{o1}
\fmfv{lab=$q_m$,l.angle=0}{o2}
\fmfv{lab=$q_i$,l.angle=180}{i1}
\fmfv{lab=$q_j$,l.angle=180}{i2}
\end{fmfgraph*}
\end{fmffile}


==> Fdiagrams/ttscatter.tex <==

\begin{fmffile}{tt_scatter}
\begin{fmfgraph*}(200,100)

\fmfleft{i1,i2}
\fmfright{o2,o1}
  \fmf{fermion,label=$t$}{i1,v2,o2}
  \fmf{fermion,label=$t$}{i2,v1,o1}
  \fmf{boson,label=$Z,,\gamma$}{v1,v2}
  
\fmfv{lab=$\bar{u}(k)$,l.angle=0}{o1}
\fmfv{lab=$\bar{u}(k')$,l.angle=0}{o2}
\fmfv{lab=$u(p)$,l.angle=180}{i2}
\fmfv{lab=$u(p')$,l.angle=180}{i1}

\end{fmfgraph*}
\end{fmffile}


==> Fdiagrams/tttt.tex <==

\begin{fmffile}{ttttcoupl}
\begin{fmfgraph*}(80,50)

\fmfleft{i1,i2}
\fmfright{o2,o1}
  \fmf{fermion,label=$t$}{i2,v1,o1}
  \fmf{fermion,label=$t$}{i1,v1,o2}
  
\fmfv{lab=$\bar{u}(k)$,l.angle=0}{o1}
\fmfv{lab=$\bar{u}(k')$,l.angle=0}{o2}
\fmfv{lab=$u(p)$,l.angle=180}{i2}
\fmfv{lab=$u(p')$,l.angle=180}{i1}
\end{fmfgraph*}
\end{fmffile}


==> Fdiagrams/udud.tex <==

\begin{fmffile}{ududcoupl}
\begin{fmfgraph*}(50,50)

\fmfleft{i1,i2}
\fmfright{o2,o1}
  \fmf{fermion}{i2,v1,i1}
  \fmf{fermion}{o1,v1,o2}
  
\fmfv{lab=$U_n$,l.angle=0}{o1}
\fmfv{lab=$D_m$,l.angle=0}{o2}
\fmfv{lab=$U_i$,l.angle=180}{i1}
\fmfv{lab=$D_j$,l.angle=180}{i2}
\end{fmfgraph*}
\end{fmffile}


==> Untitled.tex <==
First of all we thank the Referee for her/his constructive criticism.

Here follow the answers to the referee's questions and modifications.
\begin{enumerate}
\item Points 1a, 1b and 1c are all correlated:
-1a We had on purpose decided not to show explicitly in the formalism some of the weights  expected as factors in the coefficients following NDA. Indeed, there is at present a relatively intense and unresolved discussion  on which weights should be expected for the coefficients of the low-energy effective Lagrangian for the case of a composite Higgs (see e.g. MANOHAR AND BUCHALLA LAST PAPERS).  The coefficients can be easily redefined by the reader if wished. Nevertheless, because of the referee's questions and for the sake of clarification, we have now added AFTER BLA BLA a paragraph discussing such weights:

PARAGRAPH:  In the Lagrangian above, Eqs. XXX, we have chosen a definition of the operator coefficients which does not  make explicit the weights expected from Naive Dimensional Analysis (NDA, REFSXXX). While the NDA rules  are known not to be applicable to the gauge and scalar kinetic and mass terms, for the corrections they would imply suppressions by factors of the goldstone boson scale $f$ versus the high energy scale $\Lambda_s$. In particular, the coefficients of all operators in Eq. (2.6) except $P_C$, as well as all operators in Eqs. 2.7, 2.8 and 2.9, would be suppressed by the factor $f^2/\Lambda_s^2= 1/(16\pi^2)$. The coefficients can be easily redefined by the reader if wished.

1b and 1c.- The previous paragraph accounts for the expected dependence on $\Lambda_s$ related to gauge fields. In what concerns the dependence on $h$, its insertions are expected to be suppressed by the goldstone boson scale as $h/f$. This is on the contrary explicitly encoded in the present formalism, as it is a useful tool to connect with the operators in the Linear realisations. This dependence appears here through the combination of the F(h) functions and the $\xi weights$ that have been explicitly extracted. The functions $F_i(h)$ stem from an initial generic dependence of the form $(h + <h>)/f= \sqrt{\xi} (f+<h>)/v $. As an illustration,  when approaching the linear regime in which $<h>\sim v$, the $F_i$ functions are defined in the text as leading to $(1+h/v)^2$, as the $\xi$-dependence has been made explicit in the Lagrangian.  We have thus completed in the text the previous paragraph with the following description:

COMPLETING PARAGRAPH ABOVE:
The insertions of the $h$ field, explicit or through generic functions, deserve a separate comment: given their goldstonic origin, they are expected to be suppressed by the goldstone boson scale as $h/f$, as it has been already specified at the beginning of page 3. This is encoded in the present formalism by the combination of the F(h) functions as defined in the text, from which the pertinent $\xi weights$ have been explicitly extracted, as they constitute a useful tool to establish the relation with the linear expansions. Consider an initial generic dependence on the $h$ field of the form $(h + <h>)/f= v/f (f+<h>)/v$: for instance in the linear regime, in which $<h>\sim v$, the $F_i$ functions are defined in the text as leading to $(1+h/v)^2$, because the functional $\xi$-dependence has been made explicit in the Lagrangian. 


\item We have corrected the model-dependent estimates of the bounds, following the referee's comments.

\item Waiting for Concha

\end{enumerate}

We have also corrected some typos, added some references, and corrected the order number of three operators, whose $\xi$ weight was not correct: old $P_20, P_18$ and $P_13$

\end{document}


